Towards Rapid Prototyping and Comparability in Active Learning for Deep Object Detection

Active learning as a paradigm in deep learning is especially important in applications involving intricate perception tasks such as object detection where labels are difficult and expensive to acquire. Development of active learning methods in such fields is highly computationally expensive and time consuming which obstructs the progression of research and leads to a lack of comparability between methods. In this work, we propose and investigate a sandbox setup for rapid development and transparent evaluation of active learning in deep object detection. Our experiments with commonly used configurations of datasets and detection architectures found in the literature show that results obtained in our sandbox environment are representative of results on standard configurations. The total compute time to obtain results and assess the learning behavior can thereby be reduced by factors of up to 14 when comparing with Pascal VOC and up to 32 when comparing with BDD100k. This allows for testing and evaluating data acquisition and labeling strategies in under half a day and contributes to the transparency and development speed in the field of active learning for object detection.

==> tables/order_boxes.tex <==
\begin{tabular}{llllll}
\toprule
{} & FRCNN VOC & FRCNN EMNIST & YOLO VOC & RET EMNIST & RET MNIST \\
\midrule
Random             &  7 & 10 &  8 & 14 &  8 \\
Entropy (sum)      &  3 &  2 &  3 &  1 &  6 \\
Entropy (avg)      &  1 &    &  1 &  5 & 13 \\
Entropy (max)      &  2 &  1 &  2 &  4 &  2 \\
MC Dropout (sum)   &  9 &  7 &  6 &  3 &  7 \\
MC Dropout (avg)   &  5 &  5 &  7 & 12 & 14 \\
MC Dropout (max)   &  8 &  9 &  5 & 10 &  9 \\
Prob.~Margin (sum) &  4 &  8 &  4 &    &  3 \\
Prob.~Margin (avg) &    &  4 &    &  7 & 12 \\
Prob.~Margin (max) &    &  6 &    &  8 &  5 \\
Mut.~Inf. (sum)    &  6 &  3 &  9 &  2 &  1 \\
Mut.~Inf. (avg)    &    &    &    &  9 & 11 \\
Mut.~Inf. (max)    &    &    &    & 11 &  4 \\
Core Set ($L^2$)   &    &    & 10 & 13 & 10 \\
\bottomrule
\end{tabular}

==> tables/order_images.tex <==
\begin{tabular}{llllll}
\toprule
{} & FRCNN VOC & FRCNN EMNIST & YOLO VOC & RET EMNIST & RET MNIST \\
\midrule
Random             &  9 & 10 &  9 & 14 & 10 \\
Entropy (sum)      &  1 &  3 &  2 &  1 &  1 \\
Entropy (avg)      &  7 &    &  6 & 11 & 14 \\
Entropy (max)      &  3 &  4 &  4 &  5 &  8 \\
MC Dropout (sum)   &  5 &  2 &  1 &  3 &  2 \\
MC Dropout (avg)   &  8 &  8 & 10 & 13 & 12 \\
MC Dropout (max)   &  6 &  5 &  3 &  8 &  9 \\
Prob.~Margin (sum) &  2 &  7 &  5 &  2 &  4 \\
Prob.~Margin (avg) &    &  9 &    &  9 & 13 \\
Prob.~Margin (max) &    &  6 &    &  4 &  6 \\
Mut.~Inf. (sum)    &  4 &  1 &  7 &  6 &  3 \\
Mut.~Inf. (avg)    &    &    &    & 12 & 11 \\
Mut.~Inf. (max)    &    &    &    & 10 &  7 \\
Core Set ($L^2$)   &    &    &  8 &  7 &  5 \\
\bottomrule
\end{tabular}

==> tables/performance_table_frcnn_emnist.tex <==
\begin{tabular}{lllll}
\toprule
{} & $\# \mathrm{Imgs} @ 0.9$ & $\# \mathrm{Boxes} @ 0.9 $ & $\mathit{AP}_{50}^* (\mathrm{Imgs})$ & $\mathit{AP}_{50}^* (\mathrm{Boxes})$ \\
\midrule
Random             &            $1099 \pm 48$ &             $3724 \pm 135$ &                    $0.695 \pm 0.005$ &                     $0.718 \pm 0.004$ \\
Entropy (sum)      &             $702 \pm 23$ &              $2958 \pm 90$ &                    $0.734 \pm 0.003$ &                     $0.736 \pm 0.003$ \\
Entropy (max)      &             $736 \pm 18$ &              $2935 \pm 60$ &                    $0.731 \pm 0.002$ &                     $0.736 \pm 0.001$ \\
Prob.~Margin (sum) &             $772 \pm 13$ &             $3121 \pm 105$ &                    $0.727 \pm 0.001$ &                     $0.732 \pm 0.002$ \\
Prob.~Margin (avg) &             $857 \pm 11$ &              $3034 \pm 27$ &                    $0.718 \pm 0.002$ &                     $0.733 \pm 0.002$ \\
Prob.~Margin (max) &             $770 \pm 24$ &              $3076 \pm 94$ &                    $0.727 \pm 0.003$ &                     $0.733 \pm 0.003$ \\
MC Dropout (sum)   &             $696 \pm 29$ &             $3096 \pm 142$ &                    $0.735 \pm 0.003$ &                     $0.732 \pm 0.004$ \\
MC Dropout (avg)   &             $838 \pm 28$ &              $3040 \pm 94$ &                    $0.718 \pm 0.004$ &                     $0.734 \pm 0.002$ \\
MC Dropout (max)   &              $763 \pm 7$ &              $3137 \pm 54$ &                    $0.728 \pm 0.002$ &                     $0.731 \pm 0.002$ \\
Mut.~Inf. (sum)    &             $693 \pm 32$ &             $2972 \pm 115$ &                    $0.736 \pm 0.003$ &                     $0.736 \pm 0.003$ \\
\bottomrule
\end{tabular}


==> tables/performance_table_frcnn_voc.tex <==
\begin{tabular}{lllll}
\toprule
{} & $\# \mathrm{Imgs} @ 0.9$ & $\# \mathrm{Boxes} @ 0.9 $ & $\mathit{AP}_{50}^* (\mathrm{Imgs})$ & $\mathit{AP}_{50}^* (\mathrm{Boxes})$ \\
\midrule
Random             &           $1294 \pm 127$ &             $3125 \pm 267$ &                    $0.700 \pm 0.007$ &                     $0.697 \pm 0.005$ \\
Entropy (sum)      &            $1030 \pm 38$ &             $2707 \pm 125$ &                    $0.717 \pm 0.003$ &                     $0.707 \pm 0.004$ \\
Entropy (avg)      &             $1192 \pm 8$ &              $2348 \pm 48$ &                    $0.703 \pm 0.004$ &                     $0.718 \pm 0.001$ \\
Entropy (max)      &            $1076 \pm 21$ &              $2618 \pm 71$ &                    $0.713 \pm 0.002$ &                     $0.706 \pm 0.004$ \\
MC Dropout (sum)   &            $1127 \pm 65$ &             $3624 \pm 192$ &                    $0.711 \pm 0.004$ &                     $0.675 \pm 0.006$ \\
MC Dropout (avg)   &            $1232 \pm 53$ &             $2954 \pm 118$ &                    $0.702 \pm 0.008$ &                     $0.697 \pm 0.008$ \\
MC Dropout (max)   &            $1144 \pm 35$ &             $3488 \pm 125$ &                    $0.710 \pm 0.006$ &                     $0.686 \pm 0.003$ \\
Prob.~Margin (sum) &            $1037 \pm 28$ &             $2712 \pm 130$ &                    $0.718 \pm 0.003$ &                     $0.706 \pm 0.005$ \\
Mut.~Inf. (sum)    &            $1080 \pm 19$ &              $3027 \pm 57$ &                    $0.714 \pm 0.002$ &                     $0.695 \pm 0.004$ \\
\bottomrule
\end{tabular}


==> tables/performance_table_ret_emnist.tex <==
\begin{tabular}{lllll}
\toprule
{} & $\# \mathrm{Imgs} @ 0.9$ & $\# \mathrm{Boxes} @ 0.9 $ & $\mathit{AP}_{50}^* (\mathrm{Imgs})$ & $\mathit{AP}_{50}^* (\mathrm{Boxes})$ \\
\midrule
Random             &            $1495 \pm 41$ &             $5094 \pm 129$ &                    $0.723 \pm 0.003$ &                     $0.738 \pm 0.004$ \\
Entropy (sum)      &             $940 \pm 26$ &             $4052 \pm 105$ &                    $0.750 \pm 0.001$ &                     $0.750 \pm 0.002$ \\
Entropy (avg)      &            $1211 \pm 65$ &             $4118 \pm 219$ &                    $0.732 \pm 0.002$ &                     $0.748 \pm 0.002$ \\
Entropy (max)      &            $1052 \pm 51$ &             $4110 \pm 238$ &                    $0.743 \pm 0.002$ &                     $0.750 \pm 0.002$ \\
MC Dropout (sum)   &            $1011 \pm 55$ &             $4105 \pm 236$ &                    $0.746 \pm 0.004$ &                     $0.749 \pm 0.003$ \\
MC Dropout (avg)   &            $1292 \pm 22$ &             $4615 \pm 103$ &                    $0.731 \pm 0.001$ &                     $0.743 \pm 0.002$ \\
MC Dropout (max)   &            $1168 \pm 62$ &             $4488 \pm 277$ &                    $0.736 \pm 0.001$ &                     $0.745 \pm 0.003$ \\
Prob.~Margin (sum) &            $1004 \pm 73$ &             $4137 \pm 316$ &                    $0.746 \pm 0.004$ &                     $0.747 \pm 0.004$ \\
Prob.~Margin (avg) &            $1171 \pm 28$ &             $4145 \pm 126$ &                    $0.736 \pm 0.002$ &                     $0.749 \pm 0.002$ \\
Prob.~Margin (max) &             $1027 \pm 6$ &              $4148 \pm 14$ &                    $0.745 \pm 0.001$ &                     $0.749 \pm 0.000$ \\
Mut.~Inf. (sum)    &            $1054 \pm 38$ &             $4088 \pm 156$ &                    $0.744 \pm 0.001$ &                     $0.750 \pm 0.002$ \\
Mut.~Inf. (avg)    &            $1251 \pm 69$ &             $4411 \pm 177$ &                    $0.732 \pm 0.001$ &                     $0.747 \pm 0.001$ \\
Mut.~Inf. (max)    &            $1178 \pm 26$ &             $4576 \pm 145$ &                    $0.740 \pm 0.002$ &                     $0.745 \pm 0.002$ \\
Core Set ($L^2$)   &            $1158 \pm 44$ &             $4946 \pm 100$ &                    $0.742 \pm 0.001$ &                     $0.741 \pm 0.003$ \\
\bottomrule
\end{tabular}


==> tables/performance_table_ret_mnist.tex <==
\begin{tabular}{lllll}
\toprule
{} & $\# \mathrm{Imgs} @ 0.9$ & $\# \mathrm{Boxes} @ 0.9 $ & $\mathit{AP}_{50}^* (\mathrm{Imgs})$ & $\mathit{AP}_{50}^* (\mathrm{Boxes})$ \\
\midrule
Random             &             $326 \pm 10$ &              $1113 \pm 56$ &                    $0.744 \pm 0.004$ &                     $0.775 \pm 0.004$ \\
Entropy (sum)      &              $220 \pm 7$ &              $1068 \pm 34$ &                    $0.780 \pm 0.003$ &                     $0.777 \pm 0.003$ \\
Entropy (avg)      &             $403 \pm 13$ &              $1165 \pm 36$ &                    $0.722 \pm 0.004$ &                     $0.769 \pm 0.002$ \\
Entropy (max)      &              $268 \pm 8$ &              $1053 \pm 46$ &                    $0.762 \pm 0.006$ &                     $0.778 \pm 0.003$ \\
MC Dropout (sum)   &              $221 \pm 6$ &              $1102 \pm 36$ &                    $0.780 \pm 0.002$ &                     $0.775 \pm 0.003$ \\
MC Dropout (avg)   &              $393 \pm 5$ &              $1206 \pm 13$ &                    $0.722 \pm 0.007$ &                     $0.764 \pm 0.005$ \\
MC Dropout (max)   &             $283 \pm 20$ &              $1131 \pm 85$ &                    $0.760 \pm 0.006$ &                     $0.771 \pm 0.006$ \\
Prob.~Margin (sum) &             $238 \pm 11$ &              $1054 \pm 32$ &                    $0.772 \pm 0.005$ &                     $0.777 \pm 0.003$ \\
Prob.~Margin (avg) &             $394 \pm 15$ &              $1156 \pm 32$ &                    $0.732 \pm 0.002$ &                     $0.772 \pm 0.005$ \\
Prob.~Margin (max) &              $267 \pm 5$ &              $1067 \pm 35$ &                    $0.764 \pm 0.002$ &                     $0.777 \pm 0.003$ \\
Mut.~Inf. (sum)    &              $235 \pm 5$ &              $1024 \pm 22$ &                    $0.774 \pm 0.004$ &                     $0.780 \pm 0.003$ \\
Mut.~Inf. (avg)    &             $365 \pm 22$ &              $1144 \pm 77$ &                    $0.738 \pm 0.006$ &                     $0.769 \pm 0.008$ \\
Mut.~Inf. (max)    &              $267 \pm 9$ &              $1054 \pm 50$ &                    $0.765 \pm 0.003$ &                     $0.778 \pm 0.006$ \\
Core Set ($L^2$)   &              $240 \pm 7$ &              $1141 \pm 42$ &                    $0.775 \pm 0.002$ &                     $0.773 \pm 0.003$ \\
\bottomrule
\end{tabular}


==> tables/performance_table_yolo_voc.tex <==
\begin{tabular}{lllll}
\toprule
{} & $\# \mathrm{Imgs} @ 0.9$ & $\# \mathrm{Boxes} @ 0.9 $ & $\mathit{AP}_{50}^* (\mathrm{Imgs})$ & $\mathit{AP}_{50}^* (\mathrm{Boxes})$ \\
\midrule
Random             &            $2238 \pm 85$ &             $5346 \pm 269$ &                    $0.701 \pm 0.003$ &                     $0.706 \pm 0.004$ \\
Entropy (sum)      &            $1732 \pm 88$ &             $4695 \pm 319$ &                    $0.715 \pm 0.004$ &                     $0.708 \pm 0.006$ \\
Entropy (avg)      &            $1861 \pm 90$ &             $4264 \pm 185$ &                    $0.708 \pm 0.004$ &                     $0.715 \pm 0.003$ \\
Entropy (max)      &            $1794 \pm 67$ &             $4635 \pm 191$ &                    $0.710 \pm 0.003$ &                     $0.709 \pm 0.002$ \\
MC Dropout (sum)   &           $1679 \pm 167$ &             $4873 \pm 364$ &                    $0.712 \pm 0.004$ &                     $0.707 \pm 0.005$ \\
MC Dropout (avg)   &           $2241 \pm 142$ &             $5158 \pm 329$ &                    $0.700 \pm 0.005$ &                     $0.703 \pm 0.004$ \\
MC Dropout (max)   &           $1786 \pm 116$ &             $4859 \pm 244$ &                    $0.713 \pm 0.003$ &                     $0.707 \pm 0.002$ \\
Prob.~Margin (sum) &            $1858 \pm 78$ &             $4787 \pm 258$ &                    $0.706 \pm 0.002$ &                     $0.705 \pm 0.001$ \\
Mut.~Inf. (sum)    &            $1884 \pm 88$ &             $5529 \pm 304$ &                    $0.705 \pm 0.002$ &                     $0.700 \pm 0.003$ \\
Core Set ($L^2$)   &           $2121 \pm 282$ &             $6857 \pm 443$ &                    $0.710 \pm 0.002$ &                     $0.685 \pm 0.003$ \\
\bottomrule
\end{tabular}

